Measurement of the inclusive isolated prompt photon cross section in $pp$ collisions at $\sqrt{s} = 8$ TeV with the ATLAS detector

A measurement of the cross section for the inclusive production of isolated prompt photons in proton-proton collisions at a centre-of-mass energy of $\sqrt{s} = 8$ TeV is presented. The measurement covers the pseudo rapidity ranges $|\eta^{\gamma}| < 1.37$ and $1.56 \leq |\eta^{\gamma}| < 2.37$ in the transverse energy range $25 < E_{\rm T}^{\gamma} < 1500$ GeV. The results are based on an integrated luminosity of 20.2 fb$^{-1}$, recorded by the ATLAS detector at the LHC. Photon candidates are identified by combining information from the calorimeters and the inner tracker. The background is subtracted using a data-driven technique, based on the observed calorimeter shower-shape variables and the deposition of hadronic energy in a narrow cone around the photon candidate. The measured cross sections are compared with leading-order and next-to-leading order perturbative QCD calculations and are found to be in a good agreement over ten orders of magnitude.

==> sections/auxiliary.tex <==



\begin{table}[h]
\begin{center}
\begin{tabular}{@{} c  c  c | c | c | c | c | c@{}}
\toprule
\textbf{Year} & \shortstack{\textbf{Integrated} \\ \textbf{Luminosity}} & \shortstack{\textbf{Range} \\ \textbf{$\ETg$ [\GeV]}}& \multicolumn{4}{c|}{\textbf{$|\etag|$ regions}} & \textbf{$\ETiso$} [\GeV] \\
\midrule
2010
 & \phantom{.} 880~$\inb$
 & \pho15--100
 & 0--0.6
 & 0.6--1.37
 & 1.52--1.81
 &
 & 3\\
2010
 & \pho\phantom{.} 35~$\ipb$
 & \pho45--400
 & 0--0.6
 & 0.6--1.37
 & 1.52--1.81
 & 1.81--2.37
 & 3\\
2011
 & \pho4.6~$\ifb$
 & \pho100--1000
 & \multicolumn{2}{c|}{0--1.37}
 & \multicolumn{2}{c|}{1.52--2.37}
 & 7\\
2012
 & 20.2~$\ifb$
 & \pho\pho25--1500
 & 0--0.6
 & 0.6--1.37
 & 1.56--1.81
 & 1.81--2.37
 & $4.8 +4.2 \times 10^{-3} \times \ETg$ \\
\bottomrule
\end{tabular}
\caption{Coverage in $\ETg$ and $|\etag|$ for all four inclusive prompt photon measurements performed with the ATLAS detector. The quoted maximum \ETg\ refers to only the most central $|\etag|$ region of each measurement.}
\label{tab_aux:phaseSpace}
\end{center}
\end{table}

\clearpage

\begin{table}
	\begin{center}
	\begin{tabular}{c c c c}
	\toprule
	Single Photon Trigger & \ETg\ range [\GeV] & Efficiency (\%)  & Integrated Luminosity \\
	\midrule
	$\ETg \geq \pho20~\GeV$ & $25 \leq \ETg < 45$ & $100.0_{-0.06}\pho$ & $\pho 4.6~\ipb$\\
	$\ETg \geq \pho40~\GeV$ & $45 \leq \ETg < 65$ & $99.8_{-0.06}^{+0.07}$ & $\phantom{0.} 58~\ipb$\\
	$\ETg \geq \pho60~\GeV$ & $65 \leq \ETg < 85$ & $99.8_{-0.06}^{+0.07}$ & $\phantom{.} 250~\ipb$\\
	$\ETg \geq \pho80~\GeV$ & $\pho 85 \leq \ETg < 105$ & $99.7_{-0.06}^{+0.07}$ & $\phantom{.} 709~\ipb$\\
	$\ETg \geq 100~\GeV$ & $105 \leq \ETg < 125$ & $99.7_{-0.06}^{+0.07}$ & $1.55~\ifb$\\
	$\ETg \geq 120~\GeV$ & $125 \leq \ETg \phantom{<000}$ & $99.6_{-0.06}^{+0.07}$ & $20.2~\ifb$\\
	\bottomrule
 	\end{tabular}
	\caption{Trigger \ETg\ ranges, efficiencies, and integrated luminosities for each trigger used in this analysis.}
	\label{tab_aux:trig}
	\end{center}
\end{table}

\begin{figure}
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/trigger_first}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/trigger_second}
  }
  \\
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/trigger_third}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/trigger_fourth}
  }
  \caption{Photon trigger efficiencies for all six trigger thresholds used in the measurement shown as a function of $\ETg$. Each efficiency is with respect to the photons satisfying the photon identification selection.}
  \label{fig_aux:triggerEff}
\end{figure}

\begin{figure}[ht]
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/SHERPA_isoEff_first}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/SHERPA_isoEff_second}
  }
  \\
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/SHERPA_isoEff_third}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/SHERPA_isoEff_fourth}
  }
  \caption{Photon isolation efficiencies (with statistical uncertainties) as a function of $\ETg$ determined in \SHERPA\ MC simulations for four different isolation requirements. This is the efficiency of a photon candidate that satisfies the identification criteria also satisfying the isolation requirement. The isolation requirements shown include the requirement used in this measurement and two from previous ATLAS measurements.}
  \label{fig_aux:isolation}
\end{figure}

\begin{figure}[ht]
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/pythia_CombinedrecoEff_first}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/pythia_CombinedrecoEff_second}
  }
  \\
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/pythia_CombinedrecoEff_third}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/pythia_CombinedrecoEff_fourth}
  }
  \caption{The photon identification efficiencies (with statistical uncertainties) as a function of $\ETg$ determined in \PYTHIA\ MC simulations, along with the separated efficiencies for unconverted and converted photons.}
  \label{fig_aux:efficiencies}
\end{figure}

\begin{figure}
  \centering
   \includegraphics[scale=0.4]{figures/pT_TotalFakeElec}\\
  \caption{Distributions of the ratio of the number of background fake photons from electrons (with statistical uncertainties), calculated using \PYTHIA, with respect to the remaining signal photons in data, shown as a function of $\ETg$.}
  \label{fig_aux:ebackground}
\end{figure}

\begin{figure}
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/ph_pT_BinByBin_first_ptDep_real}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/ph_pT_BinByBin_second_ptDep_real}
  }
  \\
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/ph_pT_BinByBin_third_ptDep_real}
  }
  \subfloat[]{
    \includegraphics[scale=0.4]{figures/ph_pT_BinByBin_fourth_ptDep_real}
  }
  \caption{The photon unfolding correction factors (with statistical uncertainties) as a function of $\ETg$ determined in \PYTHIA\ MC simulations.}
  \label{fig_aux:correction_factor}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[scale=0.8 , angle=0]{figures/data2012_pT_NLO_pdf_ratio_pt_dep}
\caption{Ratio of theory (\JETPHOX\ using four different PDF sets: CT10, MSTW2008NLO, NNPDF2.3 and HeraPDF1.5) to data for the differential cross sections as a function of $\ETg$ for the four $|\etag|$ regions. The statistical component of the uncertainty in the data is indicated by the horizontal tick marks whereas the whole error bar corresponds to the combined statistical and systematic uncertainty (the additional systematic uncertainty arising from the uncertainty in the integrated luminosity is displayed separately as a dotted line). The NLO total uncertainty from \JETPHOX\ is displayed as a band, which exceptionally for this plot excludes the PDF uncertainty and thus corresponds to the combination of the scale, $\alphas$ and hadronisation-plus-UE uncertainties. In the highest $\ETg$ interval of the $|\etag| < 0.6$ region the theoretical predictions and uncertainty are not shown as they are above the range of the figure.
}
\label{fig_aux:xSecRatioPDF}
\end{figure}

\begin{figure}[ht]
  \subfloat[]{
  \includegraphics[scale=0.8]{figures/paper_errors_1}
  }\\
  \subfloat[]{
  \includegraphics[scale=0.8]{figures/paper_errors_2}
  }\\
  \subfloat[]{
  \includegraphics[scale=0.8]{figures/paper_errors_3}
  }\\
  \subfloat[]{
  \includegraphics[scale=0.8]{figures/paper_errors_4}
  }\\
\caption{Comparison of systematic (without the luminosity uncertainty) and statistical uncertainties for all four inclusive prompt photon measurements preformed with the ATLAS detector. Split into different $|\etag|$ regions and plotted versus $\ETg$, with the caveats that the 2011 results are repeated (as it was measured in two rather than four $\etag$ ranges) and that in (c) the 2012 measurement has a different $\etag$ lower bound.}
\label{fig_aux:uncertComparison}
\end{figure}

\clearpage


The events with $\ETg >1 \TeV$ have been visually analysed, all are found to have the signatures of good proton-proton collision events. Figures~\ref{44653203} and \ref{122752008} show the event displays of the two events with the highest photon transverse energy detected.

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.18, angle=0]
    {JiveXML_205016_44653203-YX-LegoPlot-RZ-2013-12-18-14-06-13.png}
  \caption{ Event display of the event 44653203 in Run 205016. The unconverted
    photon candidate passes the identification selection and is
    reconstructed at $\ETg=1.5~\TeV$, $\eta=0.53$ and has the isolation energy
    $0.23~\GeV$. The highest energy jet has $\pt=1.3~\TeV$.
  }
  \label{44653203}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.18, angle=0]
    {JiveXML_214758_122752008-YX-LegoPlot-RZ-2013-12-18-14-04-52.png}
  \caption{ Event display of the event 122752008 in Run 214758. The unconverted
    photon candidate passes the identification selection and is
    reconstructed at $\ETg=1.3~\TeV$, $\eta=-0.48$ and has the isolation energy
    $0.64~\GeV$. The highest energy jet has $\pt=1.2~\TeV$.
  }
  \label{122752008}
\end{figure}

\clearpage

The computed theoretical $\ETg$-differential cross sections are listed in
Table~\ref{tab_jetphox_pt1}, \ref{tab_jetphox_pt2}, ~\ref{tab_jetphox_F_pt1} and ~\ref{tab_jetphox_F_pt2}. They are also shown in the distributions shown in Figures \ref{fig_aux:jetphox_uncert} and \ref{fig_aux:jetphox_alphas}.

\begin{table}[ht]
\centering
   {\small
   \input{tables/jetphox_pt1.tex}
   }
\caption{
The \JETPHOX\ CT10 inclusive prompt photon production
cross section in the most central pseudorapidity range  $|\etag|<0.6$
as a function of $\ETg$.
}
\label{tab_jetphox_pt1}
\end{table}


\begin{table}[ht]
\centering
   {\small
   \input{tables/jetphox_pt2.tex}
   }
\caption{
The \JETPHOX\ CT10 inclusive prompt photon production
cross section in the pseudorapidity range  $0.6<|\etag|<1.37$
as a function of $\ETg$.
}
\label{tab_jetphox_pt2}
\end{table}


\begin{table}[ht]
\centering
   {\small
   \input{tables/jetphox_F_pt1.tex}
   }
\caption{
The \JETPHOX\ CT10 inclusive prompt photon production
cross section in the pseudorapidity range $1.56\leq |\etag| < 1.81$
as a function of $\ETg$.
}
\label{tab_jetphox_F_pt1}
\end{table}


\begin{table}[ht]
\centering
   {\small
   \input{tables/jetphox_F_pt2.tex}
   }
\caption{
The \JETPHOX\ CT10 inclusive prompt photon production
cross section in the pseudorapidity range $1.81\leq |\etag| < 2.37$
as a function of $\ETg$.
}
\label{tab_jetphox_F_pt2}
\end{table}

\FloatBarrier

\begin{figure}[!htb]
\includegraphics[scale=0.75, angle=0]{figures/jetphox_scale_ratio.eps}
\caption{
\JETPHOX\ inclusive prompt photon production cross section PDF and scale uncertainties
in the four $|\etag|$ regions. The PDF uncertainty is shown in green, the PDF and scale uncertainties added in quadrature is shown in green and the cross section from using the PDF MSTW2008NLO is also shown for comparison. 
}
\label{fig_aux:jetphox_uncert}
\end{figure}

\begin{figure}[!htb]
\includegraphics[scale=0.75, angle=0]{figures/jetphox_alpha_ratio.eps}
\caption{
\JETPHOX\ inclusive prompt photon production $\alpha_s$ uncertainty in the four $|\etag|$ regions. 
}
\label{fig_aux:jetphox_alphas}
\end{figure}




